Classification and Adversarial examples in an Overparameterized Linear Model: A Signal Processing Perspective

State-of-the-art deep learning classifiers are heavily overparameterized with respect to the amount of training examples and observed to generalize well on "clean" data, but be highly susceptible to infinitesmal adversarial perturbations. In this paper, we identify an overparameterized linear ensemble, that uses the "lifted" Fourier feature map, that demonstrates both of these behaviors. The input is one-dimensional, and the adversary is only allowed to perturb these inputs and not the non-linear features directly. We find that the learned model is susceptible to adversaries in an intermediate regime where classification generalizes but regression does not. Notably, the susceptibility arises despite the absence of model mis-specification or label noise, which are commonly cited reasons for adversarial-susceptibility. These results are extended theoretically to a random-Fourier-sum setup that exhibits double-descent behavior. In both feature-setups, the adversarial vulnerability arises because of a phenomenon we term spatial localization: the predictions of the learned model are markedly more sensitive in the vicinity of training points than elsewhere. This sensitivity is a consequence of feature lifting and is reminiscent of Gibb's and Runge's phenomena from signal processing and functional analysis. Despite the adversarial susceptibility, we find that classification with these features can be easier than the more commonly studied "independent feature" models.

==> commands_old.tex <==
\newcommand\argmax{\operatorname*{\arg\max}}
\newcommand\argmin{\operatorname*{\arg\min}}
\newcommand{\appropto}{\mathrel{\vcenter{
  \offinterlineskip\halign{\hfil$##$\cr
    \propto\cr\noalign{\kern2pt}\sim\cr\noalign{\kern-2pt}}}}}

\newcommand\diag{\operatorname*{diag}}
\newcommand\sinc{\operatorname*{sinc}}
\newcommand\boldparfirst[1]{\noindent \textbf{#1}}
\newcommand\boldpar[1]{\vspace{1em}
\noindent \textbf{#1}}



\newlength\mylen
\newcommand\myinput[1]{%
\settowidth\mylen{\KwIn{}}%
\setlength\hangindent{\mylen}%
\hspace*{\mylen}#1\\}
\newcommand{\Xaug}{X_{\mathsf{aug}}}
\newcommand{\Xval}{X_{\mathsf{val}}}
\newcommand{\yaug}{y_{\mathsf{aug}}}
\newcommand{\E}{\mathop{\mathbb{E}}}
\newcommand{\survival}{\ensuremath{\mathsf{SU}}}
\newcommand{\contamination}{\ensuremath{\mathsf{CN}}}

% Setup - data generation
\newcommand{\xtrain}{X_{\mathsf{train}}}
\newcommand{\xtest}{X_{\mathsf{test}}}
\newcommand{\mtrain}{M_{\mathsf{train}}}
\newcommand{\strain}{S_{\mathsf{train}}}
\newcommand{\stest}{S_{\mathsf{test}}}
\newcommand{\ytrain}{y_{\mathsf{train}}}
\newcommand{\ztrain}{z_{\mathsf{train}}}
\newcommand{\phitrain}{\phi_{\mathsf{train}}}
\newcommand{\Atrain}{A_{\mathsf{train}}}
\newcommand{\Atest}{A_{\mathsf{test}}}
\newcommand{\ALifted}{\mathsf{Lift}}
\newcommand{\minNorm}{\mathsf{Min L2}}
\newcommand{\ytest}{y_{\mathsf{test}}}
\newcommand{\ztest}{z_{\mathsf{test}}}
\newcommand{\phitest}{\phi_{\mathsf{test}}}
\newcommand{\phirfs}{\phi^{\mathsf{RFS}}}
\newcommand{\phifour}{\phi^{\mathsf{F}}}
\newcommand{\avec}{\phi}
\newcommand{\learnedfunc}{f_{\coeffs}}
\newcommand{\sgn}{\ensuremath{\mathsf{sgn}}}
\newcommand{\Sigmabold}{\ensuremath{\boldsymbol{\Sigma}}}
\newcommand{\coeffs}{\ensuremath{\boldsymbol{\hat{\alpha}}}}
\newcommand{\smallcoeffs}{\ensuremath{\boldsymbol{\hat{\zeta}}}}
\newcommand{\scaledcoeffs}{\ensuremath{\boldsymbol{\hat{\beta}}}}
\newcommand{\boldalpha}{\ensuremath{\boldsymbol{\alpha}}}
\newcommand{\boldlambda}{\ensuremath{\boldsymbol{\lambda}}}
\newcommand{\boldbeta}{\ensuremath{\boldsymbol{\beta}}}
\newcommand{\boldzeta}{\ensuremath{\boldsymbol{\zeta}}}




%New notions of margin
\newcommand{\pointwisemargin}{\gamma_{\mathsf{pw}}}
\newcommand{\nativemargin}{\ensuremath{\gamma_{\mathsf{native}}}}
\newcommand{\gradweightedmargin}{\ensuremath{\gamma_{\mathsf{GW}}}}

%Adhyyan - Ridge and SVM Stuff
\newcommand{\what}{\hat{w}_{svm}}
\newcommand{\re}{\mathbb{R}}
\newcommand{\R}{\mathbb{R}}

\newcommand{\lambar}{\vec{\lambda}}
\newcommand{\argmintwo}{\underset{\lambar, \Lambda}{argmin}}
\newcommand{\I}{\mathbb{I}}


%Adhyyan
\newcommand{\lambdabold}{\ensuremath{\mu}}
\newcommand{\Kmatrix}{\ensuremath{K}}
\newcommand{\invKmatrix}{\ensuremath{K}^{-1}}
\newcommand{\Ibold}{\ensuremath{\mathbf{I}}}
\newcommand{\Ebold}{\ensuremath{\mathbf{E}}}
\newcommand{\Ubold}{\ensuremath{\mathbf{U}}}
\newcommand{\Qbold}{\ensuremath{\mathbf{Q}}}
\newcommand{\Ybold}{\ensuremath{Y}}
\newcommand{\Jbold}{\ensuremath{\mathbf{J}}}

\newcommand{\JboldTruncated}{\ensuremath{\tilde{\mathbf{J}}}}

\newcommand{\lambdaoptsvm}{\ensuremath{\mu^*}}
\newcommand{\lambdaunconstrained}{\ensuremath{\widetilde{\mu}^*}}
\newcommand{\vecones}{\ensuremath{\mathbf{1}}}

%Adhyyan
\newcommand{\xtrue}{X_{true}}
\newcommand{\xtrash}{X_{alias}}
\newcommand{\wtrue}{w_{true}}
\newcommand{\wtrash}{w_{alias}}
\newcommand{\wtildetrash}{\widetilde{w}_{alias}}
\newcommand{\an}[1]{{\color{red} Adhyyan: #1}}
\newcommand{\vm}[1]{{\color{blue} Vidya: #1}}



%Adhyyan - adv_examples.tex
\newcommand{\nativej}{\gamma_{native}^j}
\newcommand{\native}{\gamma_{native}}
\newcommand{\nativehatj}{\hat{\gamma}_{native}^j}
\newcommand{\nativehat}{\hat{\gamma}_{native}}
\newcommand{\nativehatmodel}{\hat{\Gamma}_{native}}
\newcommand{\G}{\textbf{J}}
\newcommand{\Loss}{\mathcal{L}}
\newcommand{\aveci}{\ensuremath{\boldsymbol{\phi_i}}}
\newcommand{\phibold}{\ensuremath{\boldsymbol{\phi}}}
\newcommand{\Mbold}{\ensuremath{\mathbf{M}}}
\newcommand{\PertSet}{\mathcal{X}}
\newcommand{\learnedPredictor}{\falphahat}
\newcommand{\trueFunction}{\ensuremath{f_{true}}}
\newcommand{\norm}[1]{\left\lVert#1\right\rVert}

%Spectrally normalized margin
\newcommand{\specComplexity}{\mathbb{R_A}}

%Adv examples
\newcommand{\classlossadv}{\ensuremath{\mathcal{C}}_{adv}}
\newcommand{\Xvec}{\ensuremath{\mathbf{X}}}
\newcommand{\XVecTilde}{\ensuremath{\tilde{x}}}

%Generalization
\newcommand{\sumjdk}{\ensuremath{\sum\limits_{j=1, j \neq \truek}^d}}
\newcommand{\regloss}{\ensuremath{\mathcal{R}}}
\newcommand{\classloss}{\ensuremath{\mathcal{C}}}
\newcommand{\reglossn}{\regloss(\alphahat_{\mathsf{real}};n)}
\newcommand{\classlossn}{\classloss(\alphahat_{\mathsf{binary}};n)}

\newcommand{\survivalb}{\ensuremath{\mathsf{SU}}}
\newcommand{\contaminationb}{\ensuremath{\mathsf{CN}}}
\newcommand{\survivalr}{\survivalb_r}
\newcommand{\contaminationr}{\contaminationb_r}
\newcommand{\survivaln}{\survival(1;n)}
\newcommand{\contaminationn}{\contamination(1;n)}
\newcommand{\survivalnreal}{\survivalb_r(1;n)}
\newcommand{\contaminationnreal}{\contaminationb_r(1;n)}
\newcommand{\wip}{\mathrm{w.p.}}
\newcommand{\truek}{\ensuremath{t}}


==> experiments.tex <==
\section{Experiments}\label{sec:simulations}

While the theorems in Section~\ref{sec:main_result} are specialized to
a caricature model for analytic tractability, their value is in the
conceptual and quantitative predictions that they make. In particular,
they predict that (a) For feature families that exhibit Gibbs-type
phenomena, adversarial examples will emerge in the near vicinity of
training points whenever the overparameterization is strong enough
that the survival of the true signal drops below a critical level; (b)
For feature families that exhibit spatial localization, the
contamination can concentrate in the near vicinity of training points
in a way that is asymptotically benign, and classification
can continue to generalize well even beyond the regime where
independent feature models predict a collapse of classification
performance due to excessive contamination. 

We test these predictions in the simple one-dimensional model of
learning by drawing the training points uniformly at random instead of
on a regular grid, and by examining the Legendre polynomial feature
family. Figure~\ref{fig:function_plots} illustrates the typical local behavior
of functions learned using overparameterized Legendre
polynomials\footnote{Legendre polynomials are a standard family of
  polynomials that have been orthonormalized relative to the uniform
  distribution on $[-1,1]$.} and both the spatial localization and
Gibbs-like overshoot is clearly visible. In fact, the qualitative
resemblance to the Dirichlet kernel illustrated in
Figure~\ref{fig:dirichletkernel} is quite strong.

Figure~\ref{fig:poppingplots} depicts the results of experiments
designed to validate the predictive power of insight (a) above. The
solid curves plot the strength of the surviving true feature in the
bi-level model as $n$ varies for different $q$ scalings of the
inductive bias towards the true feature. The black curve is a
natural theoretical prediction (detailed in the supplementary
material) for the level of survival at which the Gibbs-like overshoot
phenomenon will spawn adversarial examples next to training
points. The dashed curves plot the adversarial performance with an
adversary capable of pushing test points up to $\epsilon =
\frac{1}{n}$. In Fig.~\ref{subfig:en_reg_four}, the performance of the
regularly-spaced training case is illustrated, and as expected, the
phase transition between having ubiquitous adversarial examples and
not having them occurs exactly as the corresponding solid curve drops
below the black curve.

Fig.~\ref{subfig:en_random_four} illustrates
the performance with the same Fourier features and inductive bias, but
training points chosen uniformly at random. Notice that the phase
transition occurs more smoothly, but occurs at the same place. It is
also interesting to note what the adversarial error approaches as $n$
increases. In Fig.~\ref{subfig:en_reg_four} it approaches $1$ since
every test point is within a range $\frac{1}{n}$ of a training
point. However, in Fig.~\ref{subfig:en_random_four}, it approaches
$1-\frac{1}{e}$ because with $n$ training points drawn uniformly at
random, there is a $\frac{1}{e}$ asymptotic probability that none of
the training points will be within a range of $\frac{1}{n}$ of a
particular test point.

A similar phase transition behavior for adversarial examples is seen
in the dashed curves in Fig.~\ref{subfig:en_legendre} for Legendre
polynomial features with regularly spaced training points. The solid
curves in Fig.~\ref{subfig:en_legendre} also illustrate the continued
applicability of insight (b) above. Notice that for each of the
different $q$ values representing the strength of the inductive bias
towards recovering the true features, the classification error
decreases with increasing $n$. The solid curves in all the subplots of
Fig.~\ref{fig:error_vs_n} experimentally confirm the ``asymptotically
benign contamination'' behavior that the spatial localization bias
engenders for both the Fourier and Legendre families. As summarized in
Table~\ref{tab:results}, for the larger $q$ values an independent
random feature model would instead have the classification error
increasing with increasing $n$. 

In the supplementary material (for space reasons), we also
test the predictive power of insight (a) on a random Fourier sum model
where instead of having access to a feature lifting into cleanly
scaled distinct sinusoids, we have a large collection of random
features each of which is a random sum of distinct sinusoids, where
the weighting of each sinusoid is drawn randomly with a variance
corresponding to the scaling. This is a model in the style of ``weak
feature'' models that exhibit double descent behavior. The model
exhibits Gibbs-like overshoots and we can experimentally confirm that
this indeed spawns adversarial examples in the vicinity of training
points there as well.


% in this section we show that our findings either apply seamlessly or are very informative in a wide variety of setups of interest. We create our experimental setups by modifying aspects of our theoretical framework and show that the essence of our theorems is robust to these modifications.


\iffalse
\an{TODOS for this section:
  \begin{enumerate}
    \item Error bars
    \item RFS Bilevel plots include
    \item RFS Bilevel double-descent plot
}
\fi

\begin{figure}[htpb] \label{fig:function_plots}
  % \begin{subfigure}[]{0.49\linewidth}
  %   \centering
  %   \includegraphics[width=\textwidth]{figures/individual/fourier_grid.pdf}
  % \caption{Fourier, regularly spaced }
  % \label{subfig:fp_reg_four}
  % \end{subfigure}
  % \begin{subfigure}[]{0.49\linewidth}
  %   \centering
  %   \includegraphics[width=\textwidth]{figures/individual/fourier_uniform.pdf}
  % \caption{Fourier, randomly sampled}
  % \label{subfig:fp_random_four}
  % \end{subfigure}

  \begin{subfigure}[]{0.75\linewidth}
  \begin{center}
    \includegraphics[width=\textwidth]{figures/individual/legendre_indiv.pdf}
  \end{center}
  \caption{Legendre Features with regularly spaced training data}
  \label{subfig:fp_legendre}
  \end{subfigure}
  % \begin{subfigure}[]{0.49\linewidth}
  %   \begin{center}
  %     \includegraphics[width=\textwidth]{figures/individual/rfs_indiv.pdf}
  %   \end{center}
  %   \caption{RFS, regularly spaced}
  %   \label{subfig:fp_rfs}
  % \end{subfigure}
  \caption{\textbf{Function plots for different feature families, train sampling:} Fix $n=60, p = 2, q = 1.45$, and all parameters vary according to the bilevel scalings in Definiton~\eqref{def:bilevel_covariance}. Fix $p=2$. In each of the cases, the learned function can be seen to cross the x-axis near the training point; however, the interval of $x$ for which the function's output is negative is very small. This causes the function to do well on average but perish in the face of an adversary who has the ability to search for these small regions of misclassification.}
\end{figure}

While the theorems in Section~\ref{sec:main_result} are specialized to a caricature model, in this section we show that our findings either apply seamlessly or are very informative in a wide variety of setups of interest. We create our experimental setups by modifying aspects of our theoretical framework and show that the essence of our theorems is robust to these modifications.

\begin{figure*}[htpb]
  \label{fig:error_vs_n}
  \begin{subfigure}[]{0.33\linewidth}
    \centering
    \includegraphics[width=\textwidth]{figures/error_plots/error_regspace.pdf}
  \caption{Fourier, regularly spaced}
  \label{subfig:en_reg_four}
  \end{subfigure}
  \begin{subfigure}[]{0.33\linewidth}
    \centering
    \includegraphics[width=\textwidth]{figures/error_plots/error_unif_space.pdf}
  \caption{Fourier, uniformly sampled }
  \label{subfig:en_random_four}
  \end{subfigure}
  \begin{subfigure}[]{0.33\linewidth}
  \begin{center}

  \end{center}
  \label{subfig:en_legendre}
  \centering
  \includegraphics[width=\textwidth]{figures/error_plots/error_legendre.pdf}
   \caption{Legendre, regularly spaced }
  \end{subfigure}
  % \begin{subfigure}[]{0.49\linewidth}
  %   \begin{center}
  %   \end{center}
  %   \caption{RFS, regularly spaced}
  %   \label{subfig:en_rfs}
  % \end{subfigure}
 \caption{\textbf{Classification and adversarial risk as a function of n:} All parameters vary according to the bilevel scalings in Definiton~\eqref{def:bilevel_covariance}; Fix $p=2$ and the choice of $q$ for each curve is specified in the legend. In each of the cases, the discrepancy between the adversarial loss and classification loss is large. The classification loss is seen to decrease with $n$ while adversarial loss increases, corroborating the expectation of Theorem~\ref{thm:riskabdn}.}
\end{figure*}

\begin{figure}[htpb]
  \label{fig:poppingplots}
  \begin{subfigure}[]{0.49\linewidth}
    \centering
    \includegraphics[width=\textwidth]{figures/popoff/popoff_regspace.pdf}
  \caption{Fourier, regularly spaced}
  \label{subfig:en_reg_four}
  \end{subfigure}
  \begin{subfigure}[]{0.49\linewidth}
    \centering
    \includegraphics[width=\textwidth]{figures/popoff/popoff_uniform.pdf}
  \caption{Fourier, uniformly sampled }
  \label{subfig:en_random_four}
  \end{subfigure}
  \caption{\textbf{Illustration of phase transition in Adversarial Error as a function of $n$:} All parameters vary according to the bilevel scalings in Definiton~\eqref{def:bilevel_covariance}; Fix $p=2$ and the choice of $q$ for each curve is specified in the legend. The solid curves plot $a$ and the dashed curves represent adversarial error. From Theorem~\ref{thm:riskabdn}, we notice that when $a$ dips below a threshold value which depends on $n$, we expect the adversarial error to jump to $1$ because of the undershoot of the Direchlet Kernel crossing the horizontal axis. Here, the theory's approximate prediction for the critical $n$ is denoted by the intersection of the survival curve with the dashed black line. We can see that the actual phase transition in both cases occurs very close to this predicted value, corroborating our theory.}
\end{figure}


\paragraph{Randomly sampled training data.} The first modification we consider is to sample our training data uniformly at random instead of from a grid i.e $\xtrain[i] \sim \text{Unif}([-1, 1]), \; \forall i \in [n]$. Since the learned function in this case cannot be expressed as a simple summation of aliases, this setup is less tractable theoretically. However, we notice that the key behavior of spatial localization around training points manifests almost identically in the learned functions in Figure~\ref{subfig:fp_reg_four} and Figure~\ref{subfig:fp_random_four}, and the shape of the function around each training point still resembles the Dirichlet; Figure~\ref{subfig:en_random_four} reveals the large discrepancy between regular and adversarial classification loss. 

In Theorem~\ref{thm:riskabdn}, we learned that in the regularly spaced case, a perturbation of size $\epsilon = \frac{1}{n}$ guaranteed complete adversarial vulnerability and an asymptotic $\mathcal{C}_{adv} \to 1$ for all $q>1$. This happens because a random test point is never more than $\frac{1}{n}$ distance away from the adversarial examples spawned in a training point's immediate vicinity. However, when the spacings between training data are random, then a uniformly sampled test point will be greater than $\frac{1}{n}$ distance from all training points with probability $\frac{1}{e}$. This is why in Figure~\ref{subfig:eq_random_four} and Figure~\ref{subfig:en_random_four}, the error can be seen to asymptote around $(1 - \frac{1}{e})$ instead of $1$; a calculation of this is detailed in the Supplementary Material. \an{Reference here}

\iffalse
\begin{figure}[htpb]
  \label{fig:error_vs_q}
  \begin{subfigure}[]{0.49\linewidth}
    \centering
    \includegraphics[width=\textwidth]{figures/reg_fourier/err_vs_q.pdf}
  \caption{Fourier, regularly spaced}
  \label{subfig:eq_reg_four}
  \end{subfigure}
  \begin{subfigure}[]{0.49\linewidth}
    \centering
    \includegraphics[width=\textwidth]{figures/random_fourier/err_vs_q.pdf}
  \caption{Fourier, uniformly sampled }
  \label{subfig:eq_random_four}
  \end{subfigure}
  \begin{subfigure}[]{0.49\linewidth}
  \begin{center}

  \end{center}
  \caption{Legendre, regularly spaced }
  \label{subfig:eq_legendre}
  \centering
  \includegraphics[width=\textwidth]{figures/legendre/reg_spaced/err_vs_q.pdf}
  \end{subfigure}
  \begin{subfigure}[]{0.49\linewidth}
    \begin{center}
    \end{center}
    \caption{RFS, regularly spaced}
    \label{subfig:eq_rfs}
  \end{subfigure}
  \caption{\textbf{Illustration of the seperating regime:} Fix $n = 150, p=2$, and all parameters vary according to the bilevel scalings in Definiton~\eqref{def:bilevel_covariance}. As $q$ increases and the prior becomes worse, both adversarial and classification error increase. The convergence rate of the adversarial risk to $1$ is  $n^{q-1}$, which explains the small error values that we see for small $q$. The convergence rate of the classification risk to $1$ is $n^{p-q}$, which explains why the classification risk for the chosen finite $n$ is larger for large $q$ than small $q$.}
\end{figure}
\an{There are not too many takeaways from this figure. Could remove or move to appendix if needed. If anything, the adversarial curve starting at the origin is fishy. Or maybe put them all on the same axes?}
\fi

\paragraph{Legendre Polynomial Features.} A natural question to ask is whether the spatial localization phenomena we identify is an artifact of the choice of Fourier features. Consider the following feature-map $\phi^L(x) = [\phi^L_0(x) \ldots \phi^L_{d-1}(x)] $ defined on Legendre family of orthonormal polynomials: \[
  \phi^L_K(x) = 2^K \sum_{j=0}^K x^k {K \choose j} {\frac{K + j - 1}{2} \choose K}
.\]
From Figure~\ref{subfig:fp_legendre}, we recognize that the shape of the learned function is remarkably similar to the Fourier case. Hence, it does not come as a surprise that the scaling of error with $n$ in Figure~\ref{subfig:en_legendre} and the dependence of error on the strength of the prior in Figure~\ref{subfig:eq_legendre} is nearly identical to the Fourier case.

\paragraph{Random Features.} It is instructive to consider a setup with random features as well. The featurization defined below was inspired by the weak features \citet{} that are known to exhibit double-descent. $B$ is a bandwidth parameter that controls how many Fourier features are represented in each RFS feature, and $\gamma$ determines the strength of the true feature, similarly to the bilevel weighting in Definition~\ref{def:bilevel_covariance}.

\begin{definition}[Random Fourier Sum]
 Set the parameters
\begin{align*}
  B &:= n^p \\
  \gamma &= n^{-q} .
\end{align*}

Now, define $\Sigmabold(n,p,q)$ as the diagonal matrix with entries as:
\begin{align*}
  \lambda_j=  \begin{cases}
  \gamma B, & j = 1\\
  {\frac{(1 - \gamma)B}{B-1}}, & \text{otherwise}.
  \end{cases}
\end{align*}

Then each RFS feature $\phirfs_i (x) = \langle z_i, \phifour(x)$, where each $z_i \sim \mathcal{N}(0, \Sigma)$
\end{definition}

This featurization was designed as a bridge between our caricature theoretical model and the types of models observed in practice. It satisfies the following important behaviors observed in modern machine learning:
\begin{enumerate}
  \item This choice of featurization can be thought of as a neural network with two layers, where the first layer is trained ``lazily" by sampling from the Guassian distribution and the parameters in the second layer are chosen by the min-norm interpolator from Definition~\ref{def:minl2}; this perspective is illustrated in Figure~\ref{fig:rfs_illustrate}.
  \item Each of the RFS features can be thought of as a noisy version of the true feature since it is corrupted by contributions by the spurious high-frequency Fourier terms.When thought about from this angle, it is very reminiscent of the weak-feature models proposed by \citet{}: Figure~\ref{subfig:rfs_double_descent} shows that this setup \textbf{obeys double-descent} and benefits heavily from overparameterization.
  \item This is a canonical example of the non-robust features proposed by \citeauthor{madry} which is correlated with the true signal in expectation but not under worst-case perturbations. In fact, \citeauthor{} mention in their paper ``our theoretical framework would allow for useful non-robust features to arise as combinations of useful robust features and useless non-robust features," which is exactly analogous to the present setup. In fact, the learned function in the regularly spaced Fourier case can itself be thought of as a ``non-robust feature," similar to each of the RFS features.
\end{enumerate}

From Figure~\ref{subfig:fp_rfs}, we notice that the RFS features also exhibit a spatial localization very akin to that of the Fourier features, and the adversarial examples most often proliferate in the vicinity of training points. From Figure~\ref{subfig:en_rfs}, we notice a large discrepancy between the classification and adversarial classification curves for this reason. Figure~\ref{subfig:eq_rfs} indicates that the boundaries of the seperating regime where $\mathcal{C} \to 0$ asymptotically but $\mathcal{C}_{\text{adv}} \to 1$ are roughly where we would expect from our theory. It is our hypothesis that as $d \to \infty$, the regimes would exactly co-incide with the regularly spaced Fourier, a result that is left for future work.

The RFS family hence illustrates that the insights from the caricature model are surprisingly applicable to setups that are closer to the real-world. The non-robust features that \citeauthor{madry} indicate as the cause for the adversarial susceptibility of neural networks can be learned when there are estimation-theoretic limitations (like those in Section~\ref{sec:main_result}) in the early layers of the network -- in the RFS case, a very high $q$, which is indicative of a bad prior in the first layer, can cause the features of the second layer to be non-robust.


\begin{figure}[htpb]
  \begin{subfigure}[]{\textwidth}
  \begin{center}

  \end{center}
  \caption{RFS as a lazy neural network}
  \label{subfig:rfs_lazy_train}
  \end{subfigure}
  \begin{subfigure}[]{\textwidth}
  \begin{center}

  \end{center}
  \caption{RFS exhibits double-descent.}
  \label{subfig:rfs_double_descent}
  \end{subfigure}


 \end{figure}


==> fourier_analysis.tex <==
\begingroup
\centering
\bfseries Analysis of adversarial risk of min-L2 interpolator on Fourier features \\[0.2em]
Adhyyan Narang  \\[0.2em] \today \\[0.2em]
\hrule \par
\endgroup

\section{Notation}

\textbf{Training data:} Let $S_{\mathsf{train}} \in (\re \times \{-1, 1\})^{n}$ be our train set; we collect our training examples into matrix $\xtrain$ and labels into vector $y$. $\xtrain[i] \in \re$ is the $i_{th}$ training point, and $y[i] \in \{-1, 1\}$ is the corresponding label.  At both training and test time, the points are chosen deterministically on a grid i.e at regularly spaced intervals. For the present toy setup, the labels are are independent of covariates i.e $y = 1$ for any point $x$ at training and test time.

%Lifting
\boldpar{Weighting schemes.} In order to add an explicit inductive bias, we control our choice of featurization by using the following weighting schemes.

\begin{definition} [Simple bilevel weighting]
  This weighting is parameterized by $(d, n, a, b)$. Define $\Sigma(d, n, a, b) = diag(\lambda_1 \ldots \lambda_d)$. Here,\[
    \lambda_i = \begin{cases}
      a & i \le n, \\
      b & i > n
    \end{cases}
  .\]
\end{definition}

\boldpar{Lifting} We lift our 1-D training data to $d$ dimensions by the Fourier featurization $\phi$.
\[
  \phi(x) = [\frac{1}{\sqrt{2}}, \sin(\pi x), \cos(\pi x), \sin(2\pi x), \cos(2 \pi x) \ldots \sin(\frac{d}{2} \pi x), \cos(\frac{d}{2}\pi x)]
.\]
When $\phi$ is provided a vector in $\R^n$ as input, the lifting is performed elementwise to return a $\R^{n \times d}$ dimensional matrix. Define $\Atrain: (\R^n, \R^{d \times d}) \mapsto \R^{n \times d}$ as $\Atrain(X, \Sigma) = \Sigma \phi(X)$.

\boldpar{Testing:} For a learned function $f: \re \mapsto \{-1, 1\}$, define the classification risk as follows.\[
  \mathcal{C}(f) = \E_x \mathbb{I}[\sgn(f(x)) = \sgn(x)]
.\]
And, we define the adversarial classification risk as \[
  \mathcal{C}_{\mathsf{adv}}(f) = \E_x \max_{\XVecTilde \in \PertSet(x)} \mathbb{I}[\sgn(f(\XVecTilde)) = \sgn(\XVecTilde)]
.\]
We choose as our perturbation set in the 1d case $\{\XVecTilde: |\XVecTilde - x| \leq \epsilon \}$.

\section{Goal}

Our goal in this note is to theoretically evaluate the classification and adversarial classification risks for different choices of $a$ and $b$. We hope to reveal, in closed-form, the existence of an intermediate regime where classification works but adversarial classification does not.

\section{Step 1: From roots to the risk}

If we are provided with the roots of the learned function and it's output at a single other point, we can exactly determine it's classification output everywhere. Let $\mathcal{Z} = \{l_1, r_1 \ldots l_K, r_K\}$ be the roots of the learned function in sorted order; in the intervals $(l_i, r_i)$, it's output is negative and in the intervals $(r_i, l_{i+1})$, it's output is positive. Now, the classification risk in the interval $(-1, 1)$ can be expressed as: \[
  \mathcal{C}(f) = \frac{1}{2} \sum_{i=1}^K (r_i - l_i)
.\]

By extending each of the misclassification intervals by $\epsilon$ on either side and accounting for overlaps between the intervals, define $\widetilde{r_i} = r_i + \epsilon$ and $\widetilde{l_i} = \max(l_i - \epsilon, \widetilde{r}_{i-1})$. It is easy to verify from the expressions that $\widetilde{r_i} \geq \widetilde{l_i} \geq \widetilde{r}_{i-1}$; this implies that there are no overlaps between the intervals $\{\widetilde{l_i}, \widetilde{r_i} \}_{i=1}^K$.

Now our adversarial classification risk can be similarly evaluated as \[
  \mathcal{C}_{\mathsf{adv}}(f) = \frac{1}{2}\sum_{i=1}^K (\tilde{r_i} - \tilde{l_i})
.\]

\section{Step 2: Approximate by the sinc function}

For simplicity of notation, we assume that $d - 1$ is a multiple of $2n$. We recall from previous papers that for regularly spaced Fourier features, the learned function can be expressed as \[
  \hat{f}(x) \propto \frac{a}{\sqrt{2}} 1 + b (\cos(n\pi x) + \cos(2n\pi x) + \ldots \cos(\frac{d - 1}{2} \pi x))
.\]
\begin{figure}[htpb]
  \centering
  \includegraphics[width=0.8\textwidth]{figures/analysis/learned_function.pdf}
  \caption{\textbf{Vizualization of learned function} $n = 8, d = 24n$ and $a = 1$ and $b = \frac{1}{4}$ }.
  \label{fig:learned_func}
\end{figure}

In Figure~\ref{fig:learned_func}, we see an example of this for $a = 1$ and $b= \frac{1}{4}$. Rearranging the terms above, we have:
\begin{align*}
  \hat{f}(x) &  \propto \frac{2a - b\sqrt{2}}{2\sqrt{2}} 1 + b \left( \frac{1}{2} + \cos(n\pi x) + \cos(2n\pi x) + \ldots \cos(\frac{d - 1}{2} \pi x)) \right) \\ 
  \hat{f}(x) & \propto \frac{2a - b\sqrt{2}}{2\sqrt{2}} 1 + b g(x)
\end{align*}

The constant of proportionality here is $V = a + \frac{d}{2n} b$, which we have omitted for simplicity of notation; since this is a classification problem and only the sign of the learned function influences predictions, this constant does not influence our result.

Realize that $\hat{f}$ is periodic with period $P = \frac{2}{n}$. Let $x_t$ be one of the regularly spaced training points. Because of the periodic nature, if the risks in the interval $I = (x_t - \frac{P}{2}, x_t + \frac{P}{2})$ would be exactly equal to the risks defined in the interval $(-1, 1)$.

Now, recall the expansion of the unnormalized $\sinc$ function: $\sinc(x) = \lim_{N \mapsto \infty} \frac{1}{N} \sum_{i=1}^N \cos\left( \frac{n - 1/2}{N} x \right)$. As a consequence of this expansion, in the interval $I$, \[
 b g(x) \approx \left(\frac{b d}{2n} + \frac{3}{2}\right) \sinc \left(\frac{d - 1 + n}{2} \pi x\right) = A \sinc( f x)
.\]
\an{This $\frac{3}{2}$ above should be a $\frac{1}{2}$ I think}

We define the amplitude $A$ and frequency $f$ for notational convenience, which will be handy later.

See Figure~\ref{fig:sinc_approx} for an empirical verification of the above approximation. Substituting this back, we have \[
\hat{f}(x) \appropto \frac{2a - b\sqrt{2}}{2\sqrt{2}} 1 + b \left(\frac{d}{2n} + \frac{3}{2}\right) \sinc \left(\frac{d - 1 +  n}{2} \pi x\right)
.\]

Hence, to solve $f(x) = 0$ becomes approximately equivalent in the interval $I$ to solving
\[
- \frac{2a - b\sqrt{2}}{2\sqrt{2}} = b \left(\frac{d}{2n} + \frac{3}{2}\right) \sinc \left(\frac{d - 1 + n}{2} \pi x\right)
.\]

\begin{figure}[htpb]
  \begin{subfigure}{0.5\textwidth}
  \centering
  \includegraphics[width=0.8\textwidth]{figures/analysis/sinc_approx_zoomed_out.pdf}
  \caption{Zoomed out}
  \label{subfig:}
  \end{subfigure}
  \begin{subfigure}{0.5\textwidth}
  \centering
  \includegraphics[width=0.8\textwidth]{figures/analysis/sinc_approx_zoomed_in.pdf}
  \caption{Zoomed in to single period around the origin}
  \label{subfig:}
  \end{subfigure}

  \caption{Empirical verification of approximation of parentheses function by the sinc for $n = 8$ and $d = 6n + 1$}
  \label{fig:sinc_approx}
\end{figure}

\section{Step 3: Finding the zero crossings of the sinc}

To find the zero crossings of the learned function by solving the above, we consider individual negative lobes of the sinc function and approximate it by simpler functions.

We know that $\sinc{x} = 0$ when $x = c \pi, c \in \mathbb{Z}$. Hence, we have that $\sinc{f x} = 0$ when $x = \frac{c}{f} \pi, c \in \mathbb{Z}$. Using this, we can determine that the $i_{th}$ negative lobe is located in the interval $(\frac{\pi (2i -1)}{f}, \frac{\pi 2i}{f})$.
\iffalse
\textbf{Approximation by sinusoids} We can locally approximate $A \sin(f x) \frac{1}{f x}$ by $A \sin(f x) \frac{1}{f x_0}$ for some $x_0$ that is sufficiently close to the interval where the approximation is being considered. For each negative lobe, we choose $x_0$ to be the midpoint $\frac{2i - \frac{1}{2}}{f}$. This yields our approximation \[
  p_i(x) = -\frac{A}{f x_0} \sin(fx)
.\]

Solving for the zero crossings, we have \[
  x \in \frac{\arcsin( \frac{- c f x_0}{A} + \frac{2i -1}{f})}{f}
.\]

Putting it together we have \[
  \mathcal{Z} = \bigcup_{i=1}^{\left\lceil \frac{P}{2} f \right\rceil} \frac{\arcsin( \frac{- c f x_0}{A} + \frac{2i -1}{f})}{f}
.\]
\fi

\textbf{Approximation by quadratics} Alternatively, we can consider the quadratic that has the exact same roots and the minima as the lobe under consideration. Let the quadratic approximating the $i{th}$ lobe \[
  q_i(x) = C \left(x - \frac{2i\pi}{f}\right) \left(x - \frac{(2i - 1) \pi}{f} \right)
.\]
By choosing the above form, we have fixed the roots of the quadratic to be the same as the $i_{th}$ lobe of the sinc. Setting the value of the midpoint $x_{mid} = (2i - \frac{1}{2}) \frac{\pi}{f}$ to match the sinc lobe $g(x_{mid}) = -\frac{A}{f x_{mid}}$, we obtain:
\[
  q_i(x) = \frac{4 A f^2}{\pi^3 (2i - 0.5)} \left(x - \frac{2i\pi}{f}\right) \left(x - \frac{(2i - 1) \pi}{f} \right)
.\]
\an{Need to justify that the approximation becomes exact in the limit.}

\begin{figure}[htpb]
  \centering
  \includegraphics[width=0.8\textwidth]{figures/analysis/approx_sinc_by_sine.pdf}
  \caption{\textbf{Approximation of lobes of the sinc by sinusoids}}
  \label{fig:approx_sinc_by_sine}
\end{figure}

\begin{figure}[htpb]
  \centering
  \includegraphics[width=0.8\textwidth]{figures/analysis/approx_sinc_by_quadratics.pdf}
  \caption{\textbf{Approximation of lobes of the sinc by quadratics}}
  \label{fig:approx_sinc_by_sine}
\end{figure}


\section{Using zero-crossings to obtain expressions for the risks}
\an{c does not always have to be negative. Either use an analogous procedure to solve for $c > 0$ or justify why we are not interested in this case where classification fails.}

By finding the zeros of $q_i(x)$, we can determine the length of the misclassified region for the  $k_{th}$ lobe as \[
  m_k = \frac{ \sqrt{2} (-1 + 4k)}{b (d+n)^3} \sqrt{\frac{b(d + n)^3 [2bd + \sqrt{2}a n \pi (1 - 4k) + 2bn + \pi bn (-1 + 4k)] }{(1 - 4k)^2}}
.\]

Notice that $m_k$ will either be purely real-valued or purely imaginary. If  $m_k$ is imaginary, that means that the $k_{th}$ lobe does not induce any zero-crossings in the learned function, and should hence not contribute towards the classification risk. We see that increasing $a$ has the effect of making the argument to the square root smaller and increasing $b$ has the opposite effect of making it larger; this matches our intuition because we would expect that placing higher relative weight on the true feature should reduce the number of zero crossings of the learned function. Additionally, it can be easily checked that $m_k$ is concave in $k$. Summing over each of our lobes, we can obtain an expression for the classification risk as: \[
  \mathcal{C} = \Re[\sum_{i=1}^{\left\lceil \frac{P}{2} f \right\rceil} m_k]
.\]
In the above $\Re[\cdot]$ extracts the real part.

Moving to the adversarial classification risk, we recall that $\widetilde{r_k} = r_k + \epsilon$ and  $\widetilde{l_k} = \max(l_k - \epsilon, r_{k-1} + \epsilon)$. The max would choose $l_k - \epsilon$ when  $l_k - r_{i-k} > 2 \epsilon$. Denote $d_k = l_k - r_{k-1}$, it can be checked from substituting the roots of the quadratics that:
\begin{align*}
  d_k = & \frac{(1-4 k)}{2 b (d+n)^3} \left(2 b (d+n)^2-\sqrt{2} n \sqrt{\frac{b (d+n)^3 \left(\pi  \sqrt{2} a (1-4 k) n+2 b d+b (\pi  (4 k-1)+2) n\right)}{(n-4 k n)^2}}\right) + \\
 & \frac{-(5-4 k)}{2b (d + n)^3} \left(\sqrt{2} n \sqrt{\frac{b (d+n)^3 \left(\pi  \sqrt{2} a (5-4 k) n+2 b d+b (\pi  (4 k-5)+2) n\right)}{(5-4 k)^2 n^2}}+2 b (d+n)^2\right)
\end{align*}

Now, using the expression of $d_k$, we can write the adversarial classification risk as follows: \[
\sum_{k=1}^{\left\lceil \frac{P}{2} f \right\rceil} \begin{cases}
  m_k + 2\epsilon, & d_k > 2 \epsilon \\
  m_k + \epsilon + (d_k) - \epsilon, & d_k < 2 \epsilon
\end{cases}
.\]

Further, by setting the square root in the $m_k$ expression to $0$, we obtain the critical lobe number $k^{*}$ such that  $\forall k > k*,  m_k < 0$. We have that \[
  \label{k_star}
  k^{*} = \frac{2bd + \sqrt{2} a n \pi + (2 - \pi) bn}{4 \pi n (\sqrt{2} a - b) }
.\]
This expression will be helpful when obtaining our asymptotic theorems.
\section{Obtaining asymptotic theorem}

For each of the theorems below, let our parameters scale as $a = n^{-q}, \epsilon = \frac{2}{n}, d = n^{p}$. Because of the interpolation constraint $\frac{a}{\sqrt{2}} + b \frac{d}{2n} = 1,$ we have that $b = \frac{2n - \sqrt{2} n n^{1-q}}{n^p}$.

\begin{theorem}
  $q > 1 \iff$ $\mathcal{C}_{adv} \xrightarrow{n \to \infty} 1$
\end{theorem}

\begin{proof}
  Since the learned function is periodic with period $P = \frac{2}{n}$, if there is a zero-crossing in a single oscillation, then there will be a zero-crossing in the other oscillations as well. Since $\epsilon$ is equal to the period, a single zero-crossing implies that $\mathcal{C}_{adv} = 1$. Conversely, if there are no zero-crossings in a single period, then there will be no zero-crossings in other periods either, and $\mathcal{C}_{adv} = 0$.

  Hence, $\mathcal{C}_{adv} \xrightarrow{n \to \infty} 1$ is equivalent with the first lobe inducing a zero-crossing under the assumptions of our theorem.  This would happen if and only if the $m_1$ is real i.e the argument to the square root is positive. Substituting the scalings for each of our parameters, this condition can be written as \[
    \frac{2n - \sqrt{2}n n^{2-q}}{n^p} (2 n^{p} + 2n + 3n\pi) > 3\pi \sqrt{2} n n^{1-q}
  .\]

  Equivalently, \[
    4n^{p + 1} + 4n^2 + 6n^2 \pi > 2 \sqrt{2} n^{2 + p - q} + 3\pi\sqrt{2} n^{2 - q + p} + 2\sqrt{2} n^{3-q} + 3\sqrt{2}\pi n^{3-q}
  .\]

  For the condition to be satisfied, we require $p + 1 > 2 - q + p$, or in other words $q > 1$.
\end{proof}
\an{If we can get a scaling where regression error goes to some small constant like 0.1 instead of 0, then we can get a seperating regime between regression and adv.}

Now, we consider the case when $\epsilon = \frac{2\pi}{f}$ instead.

\begin{lemma}
 \label{lem:overlaps}
 \[
   \epsilon = \frac{2\pi}{f} \implies \forall k\le  k^*, \widetilde{r}_{k-1} = \widetilde{l_k} \text{and} \widetilde{l}_1 = 0
 .\] 
\end{lemma}
\begin{proof}
The distance between the locations of minima of any two successive lobes is exactly $\frac{2\pi}{f}$. We know that $d_k = \widetilde{l}_k - \widetilde{r}_{k-1}$ cannot be larger than this. We recall that $\widetilde{l}_k = \begin{cases}
   \widetilde{r}_{k-1},& d_k < 2\epsilon,\\
   l_k - \epsilon, & otherwise
 \end{cases}$
 Because of the magnitude of $\epsilon$, we will always hit the first case. Further, $l_1 < \frac{2\pi}{f}$ must be true because $\frac{2\pi}{f}$ is the co-ordinate of the end of the first lobe. Since $\widetilde{l_1} = \max(l_1 - \epsilon, 0)$, we will always choose  $0$.
\end{proof}

\begin{lemma}
 \label{lem:adv_expr}
 \[
 \epsilon = \frac{2\pi}{f} \implies \mathcal{C}_{adv} = \frac{k^{*} \frac{2\pi}{f}}{P/2}
 .\] 
 \end{lemma}
\begin{proof}
  By Lemma~\ref{lem:overlaps}, we have that $\forall k\le k^*, \widetilde{r}_{k-1} = \widetilde{l_k}$. Plugging into the expression for adversarial risk \[
    \mathcal{C}_{adv} = \frac{\sum_{k=1}^{k^*} \widetilde{r}_k - \widetilde{l}_k}{\frac{P}{2}} = \frac{\widetilde{r}_{k^*} - \widetilde{l}_1}{\frac{P}{2}}
  .\] 
  From Lemma~\ref{lem:overlaps}, we have that $\widetilde{l_1} = 0$. And $\widetilde{r}_{k^*}$ can be approximated asymptotically by $k^{*}\times\frac{2\pi}{f}$
  Plugging this in the above gives the desired expression. 
\end{proof}


\begin{theorem}
  As $n \to \infty$, $\mathcal{C}_{adv} \to ?$
\end{theorem}
\begin{proof}
  \iffalse
  First, recognize that when the original misclassification intervals $(l_{k-1}, r_{k-1})$ and $(l_k, r_k)$ overlap upon adversarial extension, this means that any test point within $(l_{k-1}, r_k)$ will be misclassified at test time in the presence of an adversary. Next, we realize that the $d_k = l_k - r_{k-1}$ will be maximized when both the $k_{th}$ and $(k-1)_{th}$ lobe just kiss the axis; in this case, $d_k$ will be the sum of the following 3 lengths: from $r_{k-1}$ until the end of the  $(k-1)_{th}$ lobe, the length of the positive lobe in between the $(k-1)_{th}$ and  $k_{th}$ negative lobes,  from the start of the $k_{th}$ lobe until $l_k$; hence  $d_k = \frac{1}{2f} + \frac{1}{f} + \frac{1}{2f} = \frac{2}{f} = 2 \epsilon$, and $d_k \le  2\epsilon$ will always be true for our choice of scalings whenever $m_k$ is positive.
  \fi
  From Lemma~\ref{lem:adv_expr}, we have:
\[
C_{adv} =  k^{*}\times\frac{{\frac{2\pi}{f}}}{\frac{P}{2}} + \frac{\epsilon}{\frac{P}{2}} = k^{*}\times\frac{4\pi}{P f}+ \frac{2\epsilon}{P}
.\] 
Since $\epsilon$ scales slower than $P$, the second term will always $\to 0$ and we direct our attention to the first term. Consider the scaling of $P f$.  \[
  f = \frac{\pi n^p - \pi + \pi n}{2} \approx \frac{\pi n^p}{2}
.\] 
And \[
\frac{P}{2} = \frac{1}{n}
.\] 

Since we are working in the limit as $n \to \infty$, the approximation does not affect our result. Hence, the exponent on $Pf$ is $p - 1$. Now, consider the scaling of $k^{*}$ \[
    k^* = \frac{4n - (2\sqrt{2} + \pi \sqrt{2}) n^{2-q} + (4 - 2\pi) n^{2-p} + (2 - \pi) n ^{3 - q - p}}{4\pi \sqrt{2} n^{2-q} - 8\pi n^{2-p} + 4\pi \sqrt{2} n^{3 - q - p}}
  .\]

  In the denominator, $(2-q)$ dominates when $q < p$, and $(2 - p)$ dominates otherwise. In the numerator, $1$ dominates when $q < 1$ and $(2-q)$ dominates otherwise. \[
    \mathcal{C}_{adv} = \begin{cases}
    0, & q < 1 \\
    0, & 1 < q < p \\
    1, & p < q \\
  \end{cases}
  .\]  
  \iffalse
  \[
    \mathcal{C}_{adv} = 4 \left[\frac{4n^{2-p} - (2\sqrt{2} + \pi \sqrt{2}) n^{3-p -q} + (4 - 2\pi) n^{3-2p} + (2 - \pi) n ^{4 - q - 2p}}{4\pi \sqrt{2} n^{2-q} - 8\pi n^{2-p} + 4\pi \sqrt{2} n^{3 - q - p}}  \right]
  .\]
Now, consider the following table to determine which term is dominant in the numerator and denominator. We assume that $p > 1$ is always true.
\begin{center}
  \begin{tabular}{ |c|c|c|c|c| }
     \hline
     $ q < 1$ & $q < p$ & Numerator & Denominator & Risk \\
     \hline
     $0$ & $0$ & $2 - p$ & $2 - p$ & $\frac{2}{\pi}$ \\ 
     $0$ & $1$ & $2 - p$ & $2 - q$ & $0$ \\ 
     $1$ & $0$ & Impossible & & \\ 
     $1$ & $1$ & $3 - p - q$ & $2 - q$ & $0$ \\ 
     \hline
      \end{tabular}
\end{center}
\fi
\end{proof}
\an{From the four-fold picture, we realize that this error will be exactly the same as classification unless classification error tends to some constant value.}

\begin{theorem}
  As $n \to \infty, \mathcal{C} \to $
\end{theorem}

\iffalse
\section{Loose ends with analysis}

\begin{enumerate}
  \item Prove how well the approximation holds.
  \item Use inverse sinc (??) to find the roots. Complete the steps to obtain a theorem.
  \item Extend similar analysis for labels as $\sin(x)$. The sinc approximation does not hold in this case.
\end{enumerate}

\section{Survival/Contamination perspective on Humility training}

In humility training the delta function would be \[
  f_2(x) = \left(\mu_+ - 1\right) \left[ \frac{a}{\sqrt{2}} + a \cos(nx) + a \cos(2nx) \ldots \right]
.\]

Upon adding $f(x)$ and $f_2(x)$, the weights on the true feature are $\mu_+ a$ and the weights on the aliases are \[
  \mu_+a - a + b = \mu_+ a - (a - b)
.\]

The term in parentheses is positive as well; hence, the weights on the aliases are very small. The humility trained model has low survival but very low contamination. And since only the SU/C ratio should matter for classification, it's classification performance is very good even in the presence of an adversary.

\fi


==> old_result.tex <==
\section{Adversarial Classification vs Classification}

\subsection{Step 1: From roots to the risk}

If we are provided with the roots of the learned function and it's output at a single other point, we can exactly determine it's classification output everywhere. Let $\mathcal{Z} = \{l_1, r_1 \ldots l_K, r_K\}$ be the roots of the learned function in sorted order; in the intervals $(l_i, r_i)$, it's output is negative and in the intervals $(r_i, l_{i+1})$, it's output is positive. Now, the classification risk in the interval $(-1, 1)$ can be expressed as: \[
  \mathcal{C}(f) = \frac{1}{2} \sum_{i=1}^K (r_i - l_i)
.\]

By extending each of the misclassification intervals by $\epsilon$ on either side and accounting for overlaps between the intervals, define $\widetilde{r_i} = r_i + \epsilon$ and $\widetilde{l_i} = \max(l_i - \epsilon, \widetilde{r}_{i-1})$. It is easy to verify from the expressions that $\widetilde{r_i} \geq \widetilde{l_i} \geq \widetilde{r}_{i-1}$; this implies that there are no overlaps between the intervals $\{\widetilde{l_i}, \widetilde{r_i} \}_{i=1}^K$.

Now our adversarial classification risk can be similarly evaluated as \[
  \mathcal{C}_{\mathsf{adv}}(f) = \frac{1}{2}\sum_{i=1}^K (\tilde{r_i} - \tilde{l_i})
.\]

\subsection{Step 2: Approximate by the sinc function}

For simplicity of notation, we assume that $d - 1$ is a multiple of $2n$. We recall from previous papers that for regularly spaced Fourier features, the learned function can be expressed as \[
  \hat{f}(x) \propto \frac{a}{\sqrt{2}} 1 + b (\cos(n\pi x) + \cos(2n\pi x) + \ldots \cos(\frac{d - 1}{2} \pi x))
.\]
\begin{figure}[htpb]
  \centering
  \includegraphics[width=0.8\textwidth]{figures/analysis/learned_function.pdf}
  \caption{\textbf{Vizualization of learned function} $n = 8, d = 24n$ and $a = 1$ and $b = \frac{1}{4}$ }.
  \label{fig:learned_func}
\end{figure}

In Figure~\ref{fig:learned_func}, we see an example of this for $a = 1$ and $b= \frac{1}{4}$. Rearranging the terms above, we have:
\begin{align*}
  \hat{f}(x) &  \propto \frac{2a - b\sqrt{2}}{2\sqrt{2}} 1 + b \left( \frac{1}{2} + \cos(n\pi x) + \cos(2n\pi x) + \ldots \cos(\frac{d - 1}{2} \pi x)) \right) \\ 
  \hat{f}(x) & \propto \frac{2a - b\sqrt{2}}{2\sqrt{2}} 1 + b g(x)
\end{align*}

The constant of proportionality here is $V = a + \frac{d}{2n} b$, which we have omitted for simplicity of notation; since this is a classification problem and only the sign of the learned function influences predictions, this constant does not influence our result.

Realize that $\hat{f}$ is periodic with period $P = \frac{2}{n}$. Let $x_t$ be one of the regularly spaced training points. Because of the periodic nature, if the risks in the interval $I = (x_t - \frac{P}{2}, x_t + \frac{P}{2})$ would be exactly equal to the risks defined in the interval $(-1, 1)$.

Now, recall the expansion of the unnormalized $\sinc$ function: $\sinc(x) = \lim_{N \mapsto \infty} \frac{1}{N} \sum_{i=1}^N \cos\left( \frac{n - 1/2}{N} x \right)$. As a consequence of this expansion, in the interval $I$, \[
 b g(x) \approx \left(\frac{b d}{2n} + \frac{3}{2}\right) \sinc \left(\frac{d - 1 + n}{2} \pi x\right) = A \sinc( f x)
.\]
\an{This $\frac{3}{2}$ above should be a $\frac{1}{2}$ I think}

We define the amplitude $A$ and frequency $f$ for notational convenience, which will be handy later.

See Figure~\ref{fig:sinc_approx} for an empirical verification of the above approximation. Substituting this back, we have \[
\hat{f}(x) \appropto \frac{2a - b\sqrt{2}}{2\sqrt{2}} 1 + b \left(\frac{d}{2n} + \frac{3}{2}\right) \sinc \left(\frac{d - 1 +  n}{2} \pi x\right)
.\]

Hence, to solve $f(x) = 0$ becomes approximately equivalent in the interval $I$ to solving
\[
- \frac{2a - b\sqrt{2}}{2\sqrt{2}} = b \left(\frac{d}{2n} + \frac{3}{2}\right) \sinc \left(\frac{d - 1 + n}{2} \pi x\right)
.\]

\begin{figure}[htpb]
  \begin{subfigure}{0.5\textwidth}
  \centering
  \includegraphics[width=0.8\textwidth]{figures/analysis/sinc_approx_zoomed_out.pdf}
  \caption{Zoomed out}
  \label{subfig:}
  \end{subfigure}
  \begin{subfigure}{0.5\textwidth}
  \centering
  \includegraphics[width=0.8\textwidth]{figures/analysis/sinc_approx_zoomed_in.pdf}
  \caption{Zoomed in to single period around the origin}
  \label{subfig:}
  \end{subfigure}

  \caption{Empirical verification of approximation of parentheses function by the sinc for $n = 8$ and $d = 6n + 1$}
  \label{fig:sinc_approx}
\end{figure}

\subsection{Step 3: Finding the zero crossings of the sinc}

To find the zero crossings of the learned function by solving the above, we consider individual negative lobes of the sinc function and approximate it by simpler functions.

We know that $\sinc{x} = 0$ when $x = c \pi, c \in \mathbb{Z}$. Hence, we have that $\sinc{f x} = 0$ when $x = \frac{c}{f} \pi, c \in \mathbb{Z}$. Using this, we can determine that the $i_{th}$ negative lobe is located in the interval $(\frac{\pi (2i -1)}{f}, \frac{\pi 2i}{f})$.

\textbf{Approximation by quadratics} Alternatively, we can consider the quadratic that has the exact same roots and the minima as the lobe under consideration. Let the quadratic approximating the $i{th}$ lobe \[
  q_i(x) = C \left(x - \frac{2i\pi}{f}\right) \left(x - \frac{(2i - 1) \pi}{f} \right)
.\]
By choosing the above form, we have fixed the roots of the quadratic to be the same as the $i_{th}$ lobe of the sinc. Setting the value of the midpoint $x_{mid} = (2i - \frac{1}{2}) \frac{\pi}{f}$ to match the sinc lobe $g(x_{mid}) = -\frac{A}{f x_{mid}}$, we obtain:
\[
  q_i(x) = \frac{4 A f^2}{\pi^3 (2i - 0.5)} \left(x - \frac{2i\pi}{f}\right) \left(x - \frac{(2i - 1) \pi}{f} \right)
.\]
\an{Need to justify that the approximation becomes exact in the limit.}

\iffalse
\begin{figure}[htpb]
  \centering
  \includegraphics[width=0.8\textwidth]{figures/analysis/approx_sinc_by_sine.pdf}
  \caption{\textbf{Approximation of lobes of the sinc by sinusoids}}
  \label{fig:approx_sinc_by_sine}
\end{figure}
\fi

\begin{figure}[htpb]
  \centering
  \includegraphics[width=0.8\textwidth]{figures/analysis/approx_sinc_by_quadratics.pdf}
  \caption{\textbf{Approximation of lobes of the sinc by quadratics}}
  \label{fig:approx_sinc_by_sine}
\end{figure}


\subsection{Using zero-crossings to obtain expressions for the risks}
\an{c does not always have to be negative. Either use an analogous procedure to solve for $c > 0$ or justify why we are not interested in this case where classification fails.}

By finding the zeros of $q_i(x)$, we can determine the length of the misclassified region for the  $k_{th}$ lobe as \[
  m_k = \frac{ \sqrt{2} (-1 + 4k)}{b (d+n)^3} \sqrt{\frac{b(d + n)^3 [2bd + \sqrt{2}a n \pi (1 - 4k) + 2bn + \pi bn (-1 + 4k)] }{(1 - 4k)^2}}
.\]

Notice that $m_k$ will either be purely real-valued or purely imaginary. If  $m_k$ is imaginary, that means that the $k_{th}$ lobe does not induce any zero-crossings in the learned function, and should hence not contribute towards the classification risk. We see that increasing $a$ has the effect of making the argument to the square root smaller and increasing $b$ has the opposite effect of making it larger; this matches our intuition because we would expect that placing higher relative weight on the true feature should reduce the number of zero crossings of the learned function. Additionally, it can be easily checked that $m_k$ is concave in $k$. Summing over each of our lobes, we can obtain an expression for the classification risk as: \[
  \mathcal{C} = \Re[\sum_{i=1}^{\left\lceil \frac{P}{2} f \right\rceil} m_k]
.\]
In the above $\Re[\cdot]$ extracts the real part.

\iffalse
Moving to the adversarial classification risk, we recall that $\widetilde{r_k} = r_k + \epsilon$ and  $\widetilde{l_k} = \max(l_k - \epsilon, r_{k-1} + \epsilon)$. The max would choose $l_k - \epsilon$ when  $l_k - r_{i-k} > 2 \epsilon$. Denote $d_k = l_k - r_{k-1}$, it can be checked from substituting the roots of the quadratics that:
\begin{align*}
  d_k = & \frac{(1-4 k)}{2 b (d+n)^3} \left(2 b (d+n)^2-\sqrt{2} n \sqrt{\frac{b (d+n)^3 \left(\pi  \sqrt{2} a (1-4 k) n+2 b d+b (\pi  (4 k-1)+2) n\right)}{(n-4 k n)^2}}\right) + \\
 & \frac{-(5-4 k)}{2b (d + n)^3} \left(\sqrt{2} n \sqrt{\frac{b (d+n)^3 \left(\pi  \sqrt{2} a (5-4 k) n+2 b d+b (\pi  (4 k-5)+2) n\right)}{(5-4 k)^2 n^2}}+2 b (d+n)^2\right)
\end{align*}

Now, using the expression of $d_k$, we can write the adversarial classification risk as follows: \[
\sum_{k=1}^{\left\lceil \frac{P}{2} f \right\rceil} \begin{cases}
  m_k + 2\epsilon, & d_k > 2 \epsilon \\
  m_k + \epsilon + (d_k) - \epsilon, & d_k < 2 \epsilon
\end{cases}
.\]
\fi

Further, by setting the square root in the $m_k$ expression to $0$, we obtain the critical lobe number $k^{*}$ such that  $\forall k > k*,  m_k < 0$. We have that \[
  \label{k_star}
  k^{*} = \frac{2bd + \sqrt{2} a n \pi + (2 - \pi) bn}{4 \pi n (\sqrt{2} a - b) }
.\]
This expression will be helpful when obtaining our asymptotic theorems.

\subsection{Obtaining asymptotic theorem}

For each of the theorems below, let our parameters scale as $a = n^{-q}, \epsilon = \frac{2}{n}, d = n^{p}$. Because of the interpolation constraint $\frac{a}{\sqrt{2}} + b \frac{d}{2n} = 1,$ we have that $b = \frac{2n - \sqrt{2} n n^{1-q}}{n^p}$.

\begin{theorem}
  $q > 1 \iff$ $\mathcal{C}_{adv} \xrightarrow{n \to \infty} 1$
\end{theorem}

\begin{proof}
  Since the learned function is periodic with period $P = \frac{2}{n}$, if there is a zero-crossing in a single oscillation, then there will be a zero-crossing in the other oscillations as well. Since $\epsilon$ is equal to the period, a single zero-crossing implies that $\mathcal{C}_{adv} = 1$. Conversely, if there are no zero-crossings in a single period, then there will be no zero-crossings in other periods either, and $\mathcal{C}_{adv} = 0$.

  Hence, $\mathcal{C}_{adv} \xrightarrow{n \to \infty} 1$ is equivalent with the first lobe inducing a zero-crossing under the assumptions of our theorem.  This would happen if and only if the $m_1$ is real i.e the argument to the square root is positive. Substituting the scalings for each of our parameters, this condition can be written as \[
    \frac{2n - \sqrt{2}n n^{2-q}}{n^p} (2 n^{p} + 2n + 3n\pi) > 3\pi \sqrt{2} n n^{1-q}
  .\]

  Equivalently, \[
    4n^{p + 1} + 4n^2 + 6n^2 \pi > 2 \sqrt{2} n^{2 + p - q} + 3\pi\sqrt{2} n^{2 - q + p} + 2\sqrt{2} n^{3-q} + 3\sqrt{2}\pi n^{3-q}
  .\]

  For the condition to be satisfied, we require $p + 1 > 2 - q + p$, or in other words $q > 1$.
\end{proof}
\an{If we can get a scaling where regression error goes to some small constant like 0.1 instead of 0, then we can get a seperating regime between regression and adv.}

Now, we consider the case when $\epsilon = \frac{2\pi}{f}$ instead.

\begin{lemma}
 \label{lem:overlaps}
 \[
   \epsilon = \frac{2\pi}{f} \implies \forall k\le  k^*, \widetilde{r}_{k-1} = \widetilde{l_k} \text{and} \widetilde{l}_1 = 0
 .\] 
\end{lemma}
\begin{proof}
The distance between the locations of minima of any two successive lobes is exactly $\frac{2\pi}{f}$. We know that $d_k = \widetilde{l}_k - \widetilde{r}_{k-1}$ cannot be larger than this. We recall that $\widetilde{l}_k = \begin{cases}
   \widetilde{r}_{k-1},& d_k < 2\epsilon,\\
   l_k - \epsilon, & otherwise
 \end{cases}$
 Because of the magnitude of $\epsilon$, we will always hit the first case. Further, $l_1 < \frac{2\pi}{f}$ must be true because $\frac{2\pi}{f}$ is the co-ordinate of the end of the first lobe. Since $\widetilde{l_1} = \max(l_1 - \epsilon, 0)$, we will always choose  $0$.
\end{proof}

\begin{lemma}
 \label{lem:adv_expr}
 \[
 \epsilon = \frac{2\pi}{f} \implies \mathcal{C}_{adv} = \frac{k^{*} \frac{2\pi}{f}}{P/2}
 .\] 
 \end{lemma}
\begin{proof}
  By Lemma~\ref{lem:overlaps}, we have that $\forall k\le k^*, \widetilde{r}_{k-1} = \widetilde{l_k}$. Plugging into the expression for adversarial risk \[
    \mathcal{C}_{adv} = \frac{\sum_{k=1}^{k^*} \widetilde{r}_k - \widetilde{l}_k}{\frac{P}{2}} = \frac{\widetilde{r}_{k^*} - \widetilde{l}_1}{\frac{P}{2}}
  .\] 
  From Lemma~\ref{lem:overlaps}, we have that $\widetilde{l_1} = 0$. And $\widetilde{r}_{k^*}$ can be approximated asymptotically by $k^{*}\times\frac{2\pi}{f}$
  Plugging this in the above gives the desired expression. 
\end{proof}


\begin{theorem}
  As $n \to \infty$, $\mathcal{C}_{adv} \to ?$
\end{theorem}
\begin{proof}
  From Lemma~\ref{lem:adv_expr}, we have:
\[
C_{adv} =  k^{*}\times\frac{{\frac{2\pi}{f}}}{\frac{P}{2}} + \frac{\epsilon}{\frac{P}{2}} = k^{*}\times\frac{4\pi}{P f}+ \frac{2\epsilon}{P}
.\] 
Since $\epsilon$ scales slower than $P$, the second term will always $\to 0$ and we direct our attention to the first term. Consider the scaling of $P f$.  \[
  f = \frac{\pi n^p - \pi + \pi n}{2} \approx \frac{\pi n^p}{2}
.\] 
And \[
\frac{P}{2} = \frac{1}{n}
.\] 

Since we are working in the limit as $n \to \infty$, the approximation does not affect our result. Hence, the exponent on $Pf$ is $p - 1$. Now, consider the scaling of $k^{*}$ \[
    k^* = \frac{4n - (2\sqrt{2} + \pi \sqrt{2}) n^{2-q} + (4 - 2\pi) n^{2-p} + (2 - \pi) n ^{3 - q - p}}{4\pi \sqrt{2} n^{2-q} - 8\pi n^{2-p} + 4\pi \sqrt{2} n^{3 - q - p}}
  .\]

  In the denominator, $(2-q)$ dominates when $q < p$, and $(2 - p)$ dominates otherwise. In the numerator, $1$ dominates when $q < 1$ and $(2-q)$ dominates otherwise. \[
    \mathcal{C}_{adv} = \begin{cases}
    0, & q < 1 \\
    0, & 1 < q < p \\
    1, & p < q \\
  \end{cases}
  .\]  

  \end{proof}
\an{From the four-fold picture, we realize that this error will be exactly the same as classification unless classification error tends to some constant value.}

\begin{theorem}
  As $n \to \infty, \mathcal{C} \to $
\end{theorem}


